Imperative Functional Programs that Explain their Work

Program slicing provides explanations that illustrate how program outputs were produced from inputs. We build on an approach introduced in prior work by Perera et al., where dynamic slicing was defined for pure higher-order functional programs as a Galois connection between lattices of partial inputs and partial outputs. We extend this approach to imperative functional programs that combine higher-order programming with references and exceptions. We present proofs of correctness and optimality of our approach and a proof-of-concept implementation and experimental evaluation.

==> app/extra-features.tex <==
\section{Additional features}

\begin{figure}[H]
\[\begin{array}{lrcl}
\textbf{Expression} 
& e 
& ::= 
& ... \mid \ttrue \mid \tfalse 
\\

\textbf{Computation} 
& M, N 
& ::= 
& ... \mid \tif{e}{M}{M} 
\\

\textbf{Value} 
& u, v 
& ::=
& ... \mid \ttrue \mid \tfalse 
\\

\textbf{Trace}
& T 
& ::= 
& ... \mid \tifThen{t}{T} \mid \tifElse{t}{T}
\end{array}\]
\caption{Additional syntax}
\end{figure}

\begin{figure}[H]
\fbox{$\rho, e \eval v$}
\begin{mathpar}
\small
\inferrule*
{
	\strut	
}
{	
	\derives{\ttrue}{\rho,\mu, \ttrue \eval \ttrue}
}
%
\and
%
\inferrule*
{
	\strut	
}
{	
	\derives{\tfalse}{\rho,\mu, \tfalse \eval \tfalse}
}
\end{mathpar}
\\[2mm]
\fbox{$\rho, \mu, M \eval \mu', R$}
\begin{mathpar}
\small
\inferrule*
{
  	\rho,\mu, e \eval \ttrue
  	\\
  	\derives{T}{\rho,\mu, M \eval \mu', R}
}
{
  	\derives{\tifThen{e}{T}}{\rho,\mu, \tif{e}{M}{M'} \eval \mu', R}
}
%
\and
%
\inferrule*
{
  	\derives{t}{\rho,\mu, e \eval \tfalse}
  	\\
  	\derives{T}{\rho,\mu, M' \eval \mu', R}
}
{
  	\derives{\tifElse{t}{T}}{\rho,\mu, \tif{e}{M}{M'} \eval \mu', R}
}
\end{mathpar}
\caption{Big-step semantics for booleans}
\end{figure}

\begin{figure}[H]
\fbox{$\mu, R, T \bwd \rho, \mu', M$}
\begin{mathpar}
\small
\inferrule*[
	%left={B-IfThen}, 
	right={$M \neq \Hole$}
]
{
	\mu, R, T \bwd \rho, \mu', M
	\\
	\ttrue, t \bwd \rho', \mu^\twoPrime, e
}
{
	\mu, R, \tifThen{t}{T} 
	\bwd
	\rho \join \rho', \mu' \join \mu^\twoPrime, \tif{e}{M}{\Hole}	
}
%
\and
%
\inferrule*[
	right={$e \neq \Hole$}
]
{
	\mu, \Hole, T \bwd \Hole, \mu', \Hole
	\\
	\Hole, t \bwd \rho, \mu^\twoPrime, e
}
{
	\mu, \Hole, \tifThen{t}{T} 
	\bwd
	\rho, \mu' \join \mu^\twoPrime, \tif{e}{\Hole}{\Hole}	
}
%
\and
%
\inferrule*[
	%left={B-$\Hole$-IfThen}
]
{
	\mu, \Hole, T \bwd \Hole, \mu', \Hole
}
{
	\mu, \Hole, \tifThen{t}{T} 
	\bwd
	\Hole, \mu', \Hole
}
\end{mathpar}
\caption{Backward slicing for booleans}
\end{figure}

\begin{figure}[H]
\fbox{$\mu, R, T \bwd \rho, \mu', M$}
\begin{mathpar}
\small
\inferrule*[
	%left={B-IfThen}, 
	right={$M \neq \Hole$}
]
{
	\mu, R, T \bwd \rho, \mu', M
	\\
	\ttrue, t \bwd \rho', \mu^\twoPrime, e
}
{
	\mu, R, \tifThen{t}{T} 
	\bwd
	\rho \join \rho', \mu' \join \mu^\twoPrime, \tif{e}{M}{\Hole}	
}
%
\and
%
\inferrule*[
	right={$e \neq \Hole$}
]
{
	\mu, \Hole, T \bwd \Hole, \mu', \Hole
	\\
	\Hole, t \bwd \rho, \mu^\twoPrime, e
}
{
	\mu, \Hole, \tifThen{t}{T} 
	\bwd
	\rho, \mu' \join \mu^\twoPrime, \tif{e}{\Hole}{\Hole}	
}
%
\and
%
\inferrule*[
	%left={B-$\Hole$-IfThen}
]
{
	\mu, \Hole, T \bwd \Hole, \mu', \Hole
}
{
	\mu, \Hole, \tifThen{t}{T} 
	\bwd
	\Hole, \mu', \Hole
}
\end{mathpar}
\caption{Backward slicing for booleans}
\end{figure}


==> fig/slicing-bwd-hybrid.tex <==
\begin{figure}
\begin{ruleblock}{\mu, R, T \bwd \rho, \mu', M, U}
\inferrule*[
	%left={B-Hole}
]
{
        \Ell = \writes(T)
	\\
        \mu \antirestrict \Ell = \mu
}
{
	\mu, \rret~\Hole, T
	\bwd 
	\Hole, \mu, \Hole, \trhole{\Ell}
}
%
\and
\inferrule*[
	%left={B-Hole}
]
{
        \Ell = \writes(T)
	\\
        \mu \antirestrict \Ell = \mu
}
{
	\mu, \Hole, T
	\bwd 
	\Hole, \mu, \Hole, \tchole{\Ell}
}
%
\and
%
\inferrule*[
	%left={B-Ret}
]
{
	R \join \rret{\Hole} = \rret{v}\\
        v, e \bwd \rho,  e'
}
{
	\mu, R, \tret{e} 
	\bwd
	\rho, \mu, \tret{e'}, \tret{e'}
}
%
\and
%
\inferrule*[
	%left={B-Let}
]
{
	\mu, R, T_2 \bwd \extend{\rho_2}{x}{v}, \mu', M_2, U_2
	\\
	\mu', \rret{v}, T_1 \bwd \rho_1, \mu^\twoPrime, M_1, U_1
}
{
	\mu, R, \tletSucc{x}{T_1}{T_2} 
	\bwd
	\rho_1 \join \rho_2, \mu^\twoPrime, \tlet{x}{M_1}{M_2}, \tletSucc{x}{U_1}{U_2}
}
%
\and
%
\inferrule*
{
	\mu, R, T_1 \bwd \rho, \mu', M_1, U_1
}
{
	\mu, R, \tletFail{T_1}
	\bwd
	\rho, \mu', \tlet{x}{M_1}{\Hole}, \tletFail{U_1}
}
%
\and
%
\inferrule*
{
	\mu, R, T \bwd \extend{\rho}{x}{v}, \mu', M_1, U
	\\
	\tinl{v}, e \bwd \rho', e'
}
{
	\mu, R, \tcaseInl{e}{x}{T}{y} 
	\bwd 
	\rho \join \rho', \mu', \tcase{e'}{\tinlC{x}{M_1}}{\tinrC{y}{\Hole}}, \tcaseInl{e'}{x}{U}{y}
}
\and
%
\inferrule*
{
	\mu, R, T \bwd \extend{\rho}{y}{v}, \mu', M_2, U
	\\
	\tinr{v}, e \bwd \rho', e'
}
{
	\mu, R, \tcaseInr{e}{x}{y}{T}
	\bwd 
	\rho \join \rho', \mu', \tcase{e'}{\tinrC{x}{\Hole}}{\tinrC{y}{M_2}}, \tcaseInr{e'}{x}{y}{U}
}
%
\and
%
\inferrule*
{
	\mu, R, T 
	\bwd 
	\extend{\extend{\rho}{f}{v_1}}{x}{v_2}, \mu', M, U
    \\
	v_2, e_2 \bwd \rho_2, e_2'
	\\
	v_1 \join \tclosure{\rho}{f}{x}{M}, e_1 \bwd \rho_1, e_1'
}
{
	\mu, R, \tappBody{e_1}{e_2}{f}{x}{T} 
	\bwd 
	\rho_1 \join \rho_2, \mu', \tapp{e_1'}{e_2'}, \tappBody{e_1'}{e_2'}{f}{x}{U} 
}
%
\and
%
\inferrule*[
	%left={B-Raise}
]
{
  R \join \rraise{\Hole} = \rraise{v}\\
	v, e \bwd \rho, e'
}
{
	\mu,R, \traise{e} \bwd \rho, \mu, \traise{e'}, \traise{e'}
}
%
\and
%
\inferrule*[
	%left={B-TryFail}
]
{
	\mu, R, T_2 \bwd \extend{\rho_1}{x}{v}, \mu', M_2, U_2
	\\
	\mu', \rraise{v}, T_1 \bwd \rho_2, \mu^\twoPrime, M_1, U_1
}
{
	\mu, R, \ttryFail{T_1}{x}{T_2} 
	\bwd
	\rho _1\join \rho_2, \mu^\twoPrime, \ttry{M_1}{x}{M_2}, \ttryFail{U_1}{x}{U_2}
}
%
\and
%
\inferrule*[
	%left={B-TrySucc}
]
{
	\mu, R, T_1 \bwd \rho, \mu', M_1, U_1
}
{
	\mu, R, \ttrySucc{T_1} 
	\bwd
	\rho, \mu', \ttry{M_1}{x}{\Hole}, \ttrySucc{U_1}
}
% 
\and
%
\inferrule*[
	%left={B-Ref}
]
{
  R \sqcup \rret~\Hole = \rret~v
\\
	\mu(\ell), e \bwd \rho, e'
}
{
	\mu, R, \trefl{\ell}{e} 
	\bwd 
	\rho, \update{\mu}{\ell}{\Hole}, \tref{e'}, \trefl{\ell}{e'}
}
%
\and
%
\inferrule*[
	%left={B-Assign}
]
{
  \mu(\ell), e_2 \bwd \rho_2, e_2'
  \\
	\ell, e_1 \bwd \rho_1, e_1'
}
{
	\mu, R, \tassignl{e_1}{\ell}{e_2} 
	\bwd 
	\rho_1 \join \rho_2, 
	\update{\mu}{\ell}{\Hole}, \tassign{e_1'}{e_2'}, \tassignl{e_1'}{\ell}{e_2'}
}
%
\and
%
\inferrule*[
	%left={B-Deref}
]
{
  R \sqcup \rret~\Hole = \rret~v
  \\
  \ell, e \bwd \rho, e'
}
{
	\mu, R, \tderefl{\ell}{e} 
	\bwd 
	\rho, \mu \join \update{}{\ell}{v}, \tderef{e'}, \tderefl{\ell}{e'}
}
%
% \and
% %
% \inferrule*[
% 	%left={B-Deref}
% ]
% {
% \strut
% }
% {
% 	\mu, \Hole, \tderefl{\ell}{e} 
% 	\bwd 
% 	\Hole, \mu, \Hole, \thole{\varnothing}
% }
\end{ruleblock}
\caption{Backward slicing for computations (hybrid)}
\label{fig:slicing-bwd-hybrid}
\end{figure}


==> fig/slicing-bwd.tex <==
\begin{figure}
\begin{ruleblock}{\mu, R, T \bwd \rho, \mu', M, U}
\inferrule*
{
\mu \antirestrict \Ell = \mu}
{
   \mu, R, \thole{\Ell}{}
   \bwd 
   \Hole, \mu, \Hole, \thole{\Ell}{}
}
%
\and
%
\inferrule*[
   %left={B-Ret}
]
{
   \Ell = \writes(T) \\ \mu \antirestrict \Ell = \mu
}
{
   \mu, \Hole, T 
   \bwd 
   \Hole, \mu, \Hole, \thole{\Ell}{}
}
%
\and
%
\inferrule*[
   %left={B-Ret}
]
{
   v, e \bwd \rho,  e'
}
{
   \mu, \rret{v}, \tret{e} 
   \bwd
   \rho, \mu, \tret{e'}, \tret{e'}
}
%
\and
%
\inferrule*[
   %left={B-Let}
]
{
   \mu, R, T_2\bwd \extend{\rho_2}{x}{v}, \mu', M_2, U_2
   \\
   \mu', \rret{v}, T_1 \bwd \rho_1, \mu^\twoPrime, M_1, U_1
   \\
   M_1 \neq \Hole
}
{
   \mu, R, \tletSucc{x}{T_1}{T_2}
   \bwd
   \rho_1 \join \rho_2, \mu^\twoPrime, \tlet{x}{M_1}{M_2}, \tletSucc{x}{U_1}{U_2}
}
%
\and
%
\inferrule*
{
   \Ell = \writes(T_2) 
   \\
   \mu \antirestrict \Ell = \mu
   \\
   \mu, \Hole, T_1 \bwd \rho, \mu', M_1, U_1
   \\
   M_1 \neq \Hole
}
{
   \mu, \Hole, \tletSucc{x}{T_1}{T_2}
   \bwd
   \rho, \mu', \tlet{x}{M_1}{\Hole}, \tletSucc{x}{U_1}{\thole{\Ell}{}}
}
%
\and
%
\inferrule*
{
   \mu, R, T_1 \bwd \rho, \mu', M_1, U_1
   \\
   M_1 \neq \Hole
}
{
   \mu, R, \tletFail{T_1}
   \bwd
   \rho, \mu', \tlet{x}{M_1}{\Hole}, \tletFail{U_1}
}
%
\and
%
\inferrule*
{
   \mu, R, T \bwd \extend{\rho}{x}{v}, \mu', M_1, U
   \\
   M_1 \neq \Hole
   \\
   v, e \bwd \rho', e'
}
{
   \mu, R, \tcaseInl{e}{x}{T}{y} 
   \bwd 
   \rho \join \rho', \mu', \tcase{e'}{\tinlC{x}{M_1}}{\Hole}, \tcaseInl{e'}{x}{U}{y}
}
%
\and
%
\inferrule*
{
   \mu, R, T \bwd \extend{\rho}{y}{v}, \mu', M_2, U
   \\
   M_2 \neq \Hole
   \\
   v, e \bwd \rho', e'
}
{
   \mu, R, \tcaseInr{e}{x}{y}{T} 
   \bwd 
   \rho \join \rho', \mu', \tcase{e'}{\Hole}{\tinrC{x}{M_2}}, \tcaseInr{e'}{x}{y}{U}
}
%
\and
%
\inferrule*
{
   \mu, R, T 
   \bwd 
   \extend{\extend{\rho}{f}{v_1}}{x}{v_2}, \mu', M', U
   \\
   M' \neq \Hole
   \\
   v_2, e_2 \bwd \rho_2, e_2'
   \\
   v_1 \join \tclosure{\rho}{f}{x}{M'}, e_1 \bwd \rho_1, e_1'
}
{
   \mu, R, \tappBody{e_1}{e_2}{f}{x}{T} 
   \bwd 
   \rho_1 \join \rho_2, \mu', \tapp{e_1'}{e_2'}, \tappBody{e_1'}{e_2'}{f}{x}{U} 
}
%
\and
%
\inferrule*[
   %left={B-Raise}
]
{
   v, e \bwd \rho, e'
}
{
   \mu, \rraise{v}, \traise{e} \bwd \rho, \mu, \traise{e'}, \traise{e'}
}
%
\and
%
\inferrule*[
   %left={B-TryFail}
]
{
   \mu, R, T_2 \bwd \extend{\rho_1}{x}{v}, \mu', M_2, U_2
   \\
   \mu', \rraise{v}, T_1 \bwd \rho_2, \mu^\twoPrime, M_1, U_1
   \\
   M_1 \neq \Hole
}
{
   \mu, R, \ttryFail{T_1}{x}{T_2} 
   \bwd
   \rho _1\join \rho_2, \mu^\twoPrime, \ttry{M_1}{x}{M_2}, \ttryFail{U_1}{x}{U_2}
}
%
\and
%
\inferrule*
{
   \Ell = \writes(T)
   \\
   \mu \antirestrict \Ell = \mu
   \\
   \mu, \Hole, T_1 \bwd \rho, \mu', M_1, U_1
   \\
   M_1 \neq \Hole
}
{
   \mu, \Hole, \ttryFail{T_1}{x}{T_2} 
   \bwd
   \rho, \mu', \ttry{M_1}{x}{\Hole}, \ttryFail{U_1}{x}{\thole{\Ell}{}}
}
%
\and
%
\inferrule*[
   %left={B-TrySucc}
]
{
   \mu, R, T_1 \bwd \rho, \mu', M_1, U_1
   \\
   M_1 \neq \Hole
}
{
   \mu, R, \ttrySucc{T_1} 
   \bwd
   \rho, \mu', \ttry{M_1}{x}{\Hole}, \ttrySucc{U_1}
}
%
\and
%
\inferrule*[
   %left={B-Ref}
]
{
   (\mu(\ell), v) \neq (\Hole, \Hole)
   \\
   \mu(\ell), e \bwd \rho, e'
}
{
   \mu, \rret{v}, \trefl{\ell}{e} 
   \bwd 
   \rho, \update{\mu}{\ell}{\Hole}, \tref{e'}, \trefl{\ell}{e'}
}
%
\and
%
\inferrule*
{
   \mu(\ell) = \Hole
}
{
   \mu, \rret{\Hole}, \trefl{\ell}{e} 
   \bwd 
   \Hole, \update{\mu}{\ell}{\Hole}, \tref{\Hole}, \trefl{\ell}{\Hole}
}
%
\and
%
\inferrule*[
   %left={B-Assign}
]
{
   \mu(\ell) \neq \Hole
   \\
   \mu(\ell), e_2 \bwd \rho_2, e_2'
   \\
   \ell, e_1 \bwd \rho_1, e_1'
}
{
   \mu, v, \tassignl{e_1}{\ell}{e_2} 
   \bwd 
   \rho_1\join \rho_2, 
   \update{\mu}{\ell}{\Hole}, \tassign{e_1'}{e_2'}, \tassignl{e_1'}{\ell}{e_2'}
}
%
\and
%
\inferrule*[
   %left={B-Assign-$\Hole$}
]
{
   \mu(\ell) = \Hole
}
{
   \mu, \rret{v}, \tassignl{e_1}{\ell}{e_2}
   \bwd 
   \Hole, \mu, \tassign{\Hole}{\Hole}, \tassignl{\Hole}{\ell}{\Hole}
}
%
\and
%
\inferrule*[
   %left={B-Deref}
]
{
   v \neq \Hole
   \\
   \ell, e \bwd \rho, e'
}
{
   \mu, \rret{v}, \tderefl{\ell}{e} 
   \bwd 
   \rho, \mu \join \update{}{\ell}{v}, \tderef{e'}, \tderefl{\ell}{e'}
}
%
\and
%
\inferrule*
{
   \strut
}
{
   \mu, \rret{\Hole}, \tderefl{\ell}{e} 
   \bwd 
   \Hole, \mu, \tderef{\Hole}, \tderefl{\ell}{\Hole}
}
\end{ruleblock}
\caption{Backward slicing for computations (fine-grained)}
\label{fig:slicing-bwd}
\end{figure}



==> fig/slicing-fwd-hybrid.tex <==
\begin{figure}
\begin{ruleblock}{\mu, T \ffwd \mu',R}
\inferrule*
{
  \Ell = \writes(T)\\
  \rret = \res(T)
}
{
	\mu, T 
	\ffwd 
	\mu\antirestrict \Ell, \rret~\Hole
}
%
\and
%
\inferrule*
{
\Ell = \writes(T)\\
\rclueless =\res(T)
}
{
	\mu, T 
	\ffwd 
	\mu\antirestrict \Ell, \Hole
}
\end{ruleblock}
\begin{ruleblock}{\rho, \mu, M, T \fwd \mu', R}
\inferrule*
{
	\strut
}
{
   \rho, \mu, M, \trhole{\Ell}
   \fwd
   \mu \antirestrict \Ell, \rret~\Hole
}
%
\and
%
\inferrule*
{
	\strut
}
{
   \rho, \mu, M, \tchole{\Ell}
   \fwd
   \mu \antirestrict \Ell,\Hole
}
%
\and
%
\inferrule*{
\mu,T \ffwd \mu',R
}{
\rho,\mu,\Hole,T \fwd \mu',R
}
%
\and
%
\inferrule*[
	%left={F-Ret}
]
{
	\rho, e \fwd v
}
{
	\rho, \mu, \tret{e}, \tret{e'} 
	\fwd 
	\mu, \rret{v}
}
%
\and
%
\inferrule*[
	%left={F-Let}
]
{
	\rho, \mu, M_1, T_1 \fwd \mu', \rret{v}
	\\
	\extend{\rho}{x}{v}, \mu', M_2, T_2 \fwd \mu^\twoPrime, R
}
{
	\rho, \mu, \tlet{x}{M_1}{M_2}, \tletSucc{x}{T_1}{T_2}
	\fwd
	\mu^\twoPrime, R
}
%
\and
%
\inferrule*[
	%left={F-LetFail}
]
{
	\rho, \mu, M_1, T_1 \fwd \mu', R
}
{
	\rho, \mu, \tlet{x}{M_1}{M_2}, \tletFail{T_1}
	\fwd
	\mu', R
}
%
\and
%
\inferrule*[
	%left={F-LetSucc?}
]
{
	\rho, \mu, M_1, T_1 \fwd \mu', \Hole\\
        \mu', T_2 \ffwd \mu^\twoPrime, R
}
{
	\rho, \mu, \tlet{x}{M_1}{M_2}, \tletSucc{x}{T_1}{T_2}
	\fwd
	\mu^\twoPrime,R
}
%
\and
%
\inferrule*
{
	\rho, e \fwd \tinl{v}
	\\
	\extend{\rho}{x}{v}, \mu, M_1, T \fwd \mu', R
}
{
	\rho, \mu, \tcase{e}{\tinlC{x}{M_1}}{\tinrC{y}{M_2}}, \tcaseInl{e'}{x}{T}{y} 
	\fwd 
	\mu', R
}
%
\and
%
\inferrule*
{
	\rho, e \fwd \tinr{v}
	\\
	\extend{\rho}{y}{v}, \mu, M_2, T \fwd \mu', R
}
{
	\rho, \mu, \tcase{e}{\tinlC{x}{M_1}}{\tinrC{y}{M_2}}, \tcaseInr{e'}{x}{y}{T} 
	\fwd 
	\mu', R
}
%
\and
%
\inferrule*
{
	\rho, e \fwd \Hole\\
        \mu, T \ffwd \mu',R
}
{
  	\rho, \mu, \tcase{e}{\tinlC{x}{M_1}}{\tinrC{y}{M_2}},
        \tcaseInl{e'}{x}{T}{y}
	\fwd 
	\mu',R
}
%
\and
%
\inferrule*
{
	\rho, e \fwd \Hole\\
        \mu, T \ffwd \mu',R
}
{
  	\rho, \mu, \tcase{e}{\tinlC{x}{M_1}}{\tinrC{y}{M_2}},
        \tcaseInr{e'}{x}{y}{T}
	\fwd 
	\mu',R
}
%
\and
%
\inferrule*[
	%left={F-App}
]
{
	\rho, e_1 \fwd v_1
	\\
    v_1 = \tclosure{\rho'}{f}{x}{M}
    \\
	\rho, e_2 \fwd v_2
	\\
	\extend{\extend{\rho'}{f}{v_1}}{x}{v_2}, \mu, M, T \fwd \mu', R
}
{
	\rho, \mu, \tapp{e_1}{e_2}, \tappBody{e_1'}{e_2'}{f}{x}{T} 
	\fwd 
	\mu', R
}
%
\and
%
\inferrule*[
   %left={F-App-$\Hole$}
]
{
   \rho, e_1 \fwd \Hole\\
   \mu,T \ffwd \mu',R
}
{
   \rho, \mu, \tapp{e_1}{e_2}, \tappBody{e_1'}{e_2'}{f}{x}{T} 
   \fwd 
   \mu',R
}
%
\and
%
\inferrule*[
	%left={F-Raise}
]
{
	\rho, e\fwd v
}
{
	\rho, \mu, \traise{e}, \traise{e'} 
	\fwd 
	\mu, \rraise{v}
}
%
\and
%
\inferrule*[
	%left={F-TrySucc}
]
{
	\rho,\mu, M_1, T_1 \fwd \mu', R
}
{
	\rho, \mu, \ttry{M_1}{x}{M_2}, \ttrySucc{T_1}
	\fwd
	\mu', R
}
%
\and
%
\inferrule*[
	%left={F-TryFail}
]
{
	\rho, \mu, M_1, T_1 \fwd \mu', \rraise{v}
	\\
	\extend{\rho}{x}{v}, \mu', M_2, T_2 \fwd \mu^\twoPrime, R
}
{
	\rho, \mu, \ttry{M_1}{x}{M_2}, \ttryFail{T_1}{x}{T_2}
	\fwd
	\mu^\twoPrime, R
}
%
\and
%
\inferrule*[
	%left={F-TrySucc}
]
{
	\rho,\mu, M_1, T_1 \fwd \mu', \Hole\\
        \mu', T_2 \ffwd \mu^\twoPrime,R 
}
{
	\rho, \mu, \ttry{M_1}{x}{M_2},  \ttryFail{T_1}{x}{T_2}
	\fwd
	\mu^\twoPrime,R
}
%
\and
%
\inferrule*[
	%left={F-Ref}
]
{
	\rho, e \fwd v	
}
{
	\rho, \mu, \tref{e}, \trefl{\ell}{e'}
	\fwd
	\update{\mu}{\ell}{v}, \rret{\ell}
}
%
\and
%
\inferrule*[
	%left={F-Assign}
]
{
	\rho, e_1 \fwd \ell
	\\
	\rho, e_2 \fwd v
}
{
	\rho, \mu, \tassign{e_1}{e_2}, \tassignl{e_1'}{\ell}{e_2'} 
	\fwd
	\update{\mu}{\ell}{v}, \rret{\tunit}
}
%
\and
%
\inferrule*[
	%left={F-Assign-$\Hole$}
]
{
	\rho, e_1 \fwd \Hole
}
{
	\rho, \mu, \tassign{e_1}{e_2}, \tassignl{e_1'}{\ell}{e_2'} 
	\fwd
	\update{\mu}{\ell}{\Hole}, \rret{\Hole}
}
%
\and
%
\inferrule*[
	%left={F-Deref}
]
{
	\rho, e \fwd \ell
}
{
	\rho, \mu, \tderef{e}, \tderefl{\ell}{e'} 
	\fwd 
	\mu, \rret{\mu(\ell)}
}
%
\and
%
\inferrule*[
	%left={F-Deref-$\Hole$}
]
{
	\rho, e \fwd \Hole
}
{
	\rho, \mu, \tderef{e}, \tderefl{\ell}{e'} 
	\fwd 
	\mu, \rret{\Hole}
}
\end{ruleblock}
\caption{Forward slicing for computations (hybrid)}
\label{fig:slicing-fwd-hybrid}
\end{figure}


==> fig/slicing-fwd.tex <==
\begin{figure}
\begin{ruleblock}{\rho, \mu, M, T \fwd \mu', R}
\inferrule*
{
   \strut
}
{
   \rho, \mu, M, \thole{\Ell}{\kay}
   \fwd
   \mu \antirestrict \Ell, \Hole
}
%
\and
%
\inferrule*[
   %left={F-Ret}
]
{
   \rho, e\fwd v
}
{
   \rho, \mu, \tret{e}, \tret{e'} 
   \fwd 
   \mu, \rret{v}
}
%
\and
%
\inferrule*[
   %left={F-Let}
]
{
   \rho, \mu, M_1, T_1 \fwd \mu', \rret{v}
   \\
   \extend{\rho}{x}{v}, \mu', M_2, T_2 \fwd \mu^\twoPrime, R
}
{
   \rho, \mu, \tlet{x}{M_1}{M_2}, \tletSucc{x}{T_1}{T_2}
   \fwd
   \mu^\twoPrime, R
}
%
\and
%
\inferrule*[
   %left={F-LetFail}
]
{
   \rho, \mu, M_1, T_1 \fwd \mu', \rraise{v}
}
{
   \rho, \mu, \tlet{x}{M_1}{M_2}, \tletFail{T_1}
   \fwd
   \mu', \rraise{v}
}
%
%
\and
%
\inferrule*
{
   \rho, e \fwd \tinl{v}
   \\
   \extend{\rho}{x}{v}, \mu, M_1, T \fwd \mu', R
}
{
   \rho, \mu, \tcase{e}{\tinlC{x}{M_1}}{\tinrC{y}{M_2}}, \tcaseInl{e'}{x}{T}{y} 
   \fwd 
   \mu', R
}
%
\and
%
\inferrule*
{
   \rho, e \fwd \tinr{v}
   \\
   \extend{\rho}{y}{v}, \mu, M_2, T \fwd \mu', R
}
{
   \rho, \mu, \tcase{e}{\tinlC{x}{M_1}}{\tinrC{y}{M_2}}, \tcaseInr{e'}{x}{y}{T} 
   \fwd 
   \mu', R
}
\and
%
\inferrule*[
   %left={F-App}
]
{
   \rho, e_1 \fwd v_1
   \\
    v_1 = \tclosure{\rho'}{f}{x}{M}
    \\
   \rho, e_2 \fwd v_2
   \\
   \extend{\extend{\rho'}{f}{v_1}}{x}{v_2}, \mu, M, T \fwd \mu', R
}
{
   \rho, \mu, \tapp{e_1}{e_2}, \tappBody{e_1'}{e_2'}{f}{x}{T} 
   \fwd 
   \mu', R
}
\and
%
\inferrule*[
   %left={F-Raise}
]
{
   \rho, e\fwd v
}
{
   \rho, \mu, \traise{e}, \traise{e'} 
   \fwd 
   \mu, \rraise{v}
}
%
\and
%
\inferrule*[
   %left={F-TrySucc}
]
{
   \rho,\mu, M_1, T_1 \fwd \mu', \rret{v}
}
{
   \rho, \mu', \ttry{M_1}{x}{M_2}, \ttrySucc{T_1}
   \fwd
   \mu', \rret{v}
}
%
\and
%
\inferrule*[
   %left={F-TryFail}
]
{
   \rho, \mu, M_1, T_1 \fwd \mu', \rraise{v}
   \\
   \extend{\rho}{x}{v}, \mu', M_2, T_2 \fwd \mu^\twoPrime, R
}
{
   \rho, \mu, \ttry{M_1}{x}{M_2}, \ttryFail{T_1}{x}{T_2}
   \fwd
   \mu^\twoPrime, R
}
%
\and
%
\inferrule*[
   %left={F-Ref}
]
{
   \rho, e \fwd v 
}
{
   \rho, \mu, \tref{e}, \trefl{\ell}{e'}
   \fwd
   \update{\mu}{\ell}{v}, \rret{\ell}
}
%
\and
%
\inferrule*[
   %left={F-Assign}
]
{
   \rho, e_1 \fwd \ell
   \\
   \rho, e_2 \fwd v
}
{
   \rho, \mu, \tassign{e_1}{e_2}, \tassignl{e_1'}{\ell}{e_2'} 
   \fwd
   \update{\mu}{\ell}{v}, \rret{\tunit}
}
%
\and
%
\inferrule*[
   %left={F-Assign-$\Hole$}
]
{
   \rho, e_1\fwd \Hole
}
{
   \rho, \mu, \tassign{e_1}{e_2}, \tassignl{e_1'}{\ell}{e_2'} 
   \fwd
   \update{\mu}{\ell}{\Hole}, \rret{\tunit}
}
%
\and
%
\inferrule*[
   %left={F-Deref}
]
{
   \rho, e\fwd \ell     
}
{
   \rho, \mu, \tderef{e}, \tderefl{\ell}{e'} 
   \fwd 
   \mu, \rret{\mu(\ell)}
}
%
\and
%
\inferrule*[
   %left={F-Deref-$\Hole$}
]
{
   \rho, e \fwd \Hole      
}
{
   \rho, \mu, \tderef{e}, \tderefl{\ell}{e'} 
   \fwd 
   \mu, \rret{\Hole}
}
\end{ruleblock}
%
\crossrule
%
\begin{smathpar}
\inferrule*
{
  \Ell = \writes(T)
}
{
   \rho, \mu, \Hole, T 
   \fwd 
   \mu \antirestrict \Ell, \Hole
}
%
\and
%
\inferrule*[
   %left={F-App-$\Hole$}
]
{
   \rho, e_1 \fwd \Hole
   \\
   \Ell = \writes(T)
}
{
   \rho, \mu, \tapp{e_1}{e_2}, \tappBody{e_1'}{e_2'}{f}{x}{T} 
   \fwd 
   \mu \antirestrict \Ell, \Hole
}
%
\and
%
\inferrule*[
   %left={F-Let-$\Hole$}
]
{
   \rho, \mu, M_1, T_1 \fwd \mu', \Hole
   \\
   \Ell = \writes(T_2)
}
{
   \rho, \mu, \tlet{x}{M_1}{M_2}, \tletSucc{x}{T_1}{T_2}
   \fwd
   \mu' \antirestrict \Ell, \Hole
}
%
\and
%
\inferrule*[
   %left={F-LetFail-$\Hole$}
]
{
   \rho, \mu, M_1, T_1 \fwd \mu', \Hole
}
{
   \rho, \mu, \tlet{x}{M_1}{M_2}, \tletFail{T_1}
   \fwd
   \mu', \Hole
}
\and
%
\inferrule*[
   %left={F-TryFail-$\Hole$}
]
{
   \rho, \mu, M_1, T_1 \fwd \mu', \Hole
   \\
   \Ell = \writes(T_2)
}
{
   \rho, \mu, \ttry{M_1}{x}{M_2}, \ttryFail{T_1}{x}{T_2}
   \fwd
   \mu'\antirestrict \Ell, \Hole
}
%
\and
%
\inferrule*[
   %left={F-TrySucc-$\Hole$}
]
{
   \rho, \mu, M_1, T_1 \fwd \mu', \Hole
}
{
   \rho, \mu, \ttry{M_1}{x}{M_2}, \ttrySucc{T_1}
   \fwd
   \mu', \Hole
}
%
\and
%
\inferrule*
{
   \rho, e \fwd \Hole
   \\
   \Ell = \writes(T)
}
{
   \rho, \mu, \tcase{e}{\tinlC{x}{M_1}}{\tinrC{y}{M_2}}, \tcaseInl{e'}{x}{T}{y} 
   \fwd 
   \mu\antirestrict \Ell, \Hole
}
%
\end{smathpar}
\caption{Forward slicing for computations (fine-grained)}
\label{fig:slicing-fwd}
\end{figure}


==> full.tex <==
\def\includeapp{1}
\input{main}

